A Quantum Money Solution to the Blockchain Scalability Problem

We put forward the idea that classical blockchains and smart contracts are potentially useful primitives not only for classical cryptography, but for quantum cryptography as well. Abstractly, a smart contract is a functionality that allows parties to deposit funds, and release them upon fulfillment of algorithmically checkable conditions, and can thus be employed as a formal tool to enforce monetary incentives. In this work, we give the first example of the use of smart contracts in a quantum setting. We describe a simple hybrid classical-quantum payment system whose main ingredients are a classical blockchain capable of handling stateful smart contracts, and quantum lightning, a strengthening of public-key quantum money introduced by Zhandry (Eurocrypt'19). Our hybrid payment system employs quantum states as banknotes and a classical blockchain to settle disputes and to keep track of the valid serial numbers. It has several desirable properties: it is decentralized, requiring no trust in any single entity; payments are as quick as quantum communication, regardless of the total number of users; when a quantum banknote is damaged or lost, the rightful owner can recover the lost value.

==> arxiv upload/macros.tex <==
\ifnum\sigconf=0\usepackage{authblk}\fi \usepackage{silence} %authbulk must loaded before the silence package!!
\usepackage[modulo]{lineno}
\usepackage{amsthm,amssymb,amsfonts,latexsym,color,paralist,url,ifdraft,mathrsfs,thm-restate,comment,bbold,booktabs}





\usepackage[utf8]{inputenc} \usepackage[autostyle=false, style=english]{csquotes} \MakeOuterQuote{"}
%csquotes after inputenc
\usepackage[T1]{fontenc}
\ifnum\sigconf=0
    \usepackage[draft=false,pageanchor]{hyperref}
    \def\pagedeclaration#1{, \hyperlink{page.#1}{page\nobreakspace#1}}
    \usepackage[final]{graphicx}
\fi
 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases.
\ifdraft{\usepackage{showlabels}}{} %must be after use package{hyperref}.

%\usepackage[refpage,prefix]{nomencl} \newcommand*{\nom}[2]{#1\nomenclature{#1}{#2}} \makenomenclature
%\usepackage[displaymath,textmath,sections,graphics,floats]{preview}
%\RequirePackage{silence}
\WarningFilter{l3regex}{This package is obsolete }
\RequirePackage{etex}
\usepackage [ lambda,advantage , operators , sets , adversary , landau , probability , notions , logic ,ff, mm,primitives , events , complexity , asymptotics , keys]{cryptocode}
%the following commands are defined by crptocode. Define these ourselves if needed: \newcommand{\poly}{\mathrm{poly}} \newcommand{\prob}[1]{\Pr[ #1 ]} \newcommand{\norm}[1]{\left\| #1 \right\|} \newcommand{\RR}{\mathbb{R}} \newcommand{\FF}{\mathbb{F}} \newcommand{\CC}{\mathbb{C}} \newcommand{\NN}{\mathbb{N}}\DeclarePairedDelimiter\ceil{\lceil}{\rceil} \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\renewcommand{\verify}{\ensuremath{\mathsf{verify}}} 


%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}
\theoremstyle{plain}
  
\ifnum\sigconf=0
    \newtheorem{theorem}{Theorem}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{definition}[theorem]{Definition}
    \newtheorem{example}[theorem]{Example}
    \newtheorem{conjecture}[theorem]{Conjecture}
\fi 
  \newtheorem{claim}[theorem]{Claim}
  \newtheorem{fact}[theorem]{Fact}
  \newtheorem*{theorem*}{Theorem}
  \newtheorem*{lemma*}{Lemma}
  \newtheorem*{corollary*}{Corollary}
  \newtheorem*{proposition*}{Proposition}
  \newtheorem*{claim*}{Claim}
  
  \theoremstyle{definition}
  \newtheorem{openproblem}[theorem]{Open Problem}
  \theoremstyle{remark}
  \newtheorem{remark}[theorem]{Remark}

  \theoremstyle{plain}
  \renewcommand{\qedsymbol}{$\square$}

% ---------------------------------------------------------------------------
\ifdraft{\newcommand{\authnote}[3]{{\color{#3} {\bf  #1:} #2}}}{\newcommand{\authnote}[3]{}}
\newcommand{\note}[1]{{\color{red}#1}}
%Example for how this should be used, in main file:
%\newcommand{\onote}[1]{\authnote{Or}{#1}{blue}}


\newcommand{\CNOT}{\mathrm{CNOT}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}

\newcommand{\const}{\mathrm{const}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}
\newcommand{\ketbra}[1]{\vert #1 \rangle \langle #1 \vert}
\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle}
\newcommand{\conjugate}[1]{#1^{\dagger}}
\newcommand{\tensor}{\otimes}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\transpose}[1]{#1^{\mathsf{T}}}
\ifdraft{\linenumbers}{}

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\E}{\mathbb{E}}

%\PreviewMacro*\onote
%\PreviewMacro*\nom
%\PreviewMacro*\ifdraft
%\DeclareMathOperator*{\E}{\scalerel*{\mathbb{E}}{\textstyle\sum}}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%document specific
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage[normalem]{ulem}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\inj}{J}
\newcommand{\Es}[1]{\textsc{E}_{#1}}
\newcommand{\dset}{G}
\newcommand{\BQP}{\textsf{BQP}}
\renewcommand{\supp}{\textsc{Supp}}
\newcommand{\decrypt}{\ensuremath{\mathsf{decrypt}}}
\newcommand{\encrypt}{\ensuremath{\mathsf{encrypt}}}
\newcommand{\otr}{\ensuremath{\mathsf{OTR}}}
\newcommand{\ot}{\ensuremath{\mathsf{OT}}}
\newcommand{\ts}{\ensuremath{\mathsf{TS}}}
\newcommand{\ds}{\ensuremath{\mathsf{DS}}}
\newcommand{\tm}{\ensuremath{\mathsf{TM}}}
\newcommand{\stamp}{
 {\mathchoice
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.2ex]{RubberStamp}}
  {\includegraphics[height=0.9ex]{RubberStamp}}
 }
}
%\newcommand{\keygen}{\ensuremath{\mathsf{key\textit{-}gen}}}
\newcommand{\tokengen}{\ensuremath{\mathsf{token\textit{-}gen}}}
%\newcommand{\sign}{\ensuremath{\mathsf{sign}}}
%\newcommand{\verify}{\ensuremath{\mathsf{verify}}}


\usepackage{tikz}
\usetikzlibrary{arrows,chains,matrix,positioning,scopes}
%
\makeatletter
\tikzset{join/.code=\tikzset{after node path={%
\ifx\tikzchainprevious\pgfutil@empty\else(\tikzchainprevious)%
edge[every join]#1(\tikzchaincurrent)\fi}}}
\makeatother
%
\tikzset{>=stealth',every on chain/.append style={join},
         every join/.style={->}}
\tikzstyle{labeled}=[execute at begin node=$\scriptstyle,
   execute at end node=$]
\ifnum\sigconf=0
    \usepackage[capitalise]{cleveref} %Incompatible with showonlyrefs
\fi
\usepackage{autonum}%must be loaded after cleveref. Sometimes causes bugs. The alternative is incomaptible with cleveref:
 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases. In any case, showonlyrefs does not work with cleveref.



%Abstract:
%\newcommand{\ab}[1]{#1} \newcommand{\fv}[1]{}

%Full version:
\newcommand{\ab}[1]{} \newcommand{\fv}[1]{#1} %%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end macros
